Robust Price Optimization of Multiple Products under Interval Uncertainties

In this paper, we solve the multiple product price optimization problem under interval uncertainties of the price sensitivity parameters in the demand function. The objective of the price optimization problem is to maximize the overall revenue of the firm where the decision variables are the prices of the products supplied by the firm. We propose an approach that yields optimal solutions under different variations of the estimated price sensitivity parameters. We adopt a robust optimization approach by building a data-driven uncertainty set for the parameters, and then construct a deterministic counterpart for the robust optimization model. The numerical results show that two objectives are fulfilled: the method reflects the uncertainty embedded in parameter estimations, and also an interval is obtained for optimal prices. We also conducted a simulation study to which we compared the results of our approach. The comparisons show that although robust optimization is deemed to be conservative, the results of the proposed approach show little loss compared to those from the simulation.

==> table2.tex <==
\begin{landscape}
	\begin{center} 
%\begin{table}[!h] 
	\footnotesize   
\begin{longtable}{|l|c|rrrrrrrrrrr|r|}
	%\begin{tabular}{|c|c|c|rrrrrrrrrr|}
	\hline\hline 
	& & \multicolumn{11}{|c|}{Optimal Values} & \\
	\cline{3-13}
	Sample & & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & Decline (\%) \\
\hline
\multirow{2}{*}{S1} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{3.0711} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.992966} & {\hspace{-2mm}\scriptsize 0.986066} & {\hspace{-2mm}\scriptsize 0.979196} & {\hspace{-2mm}\scriptsize 0.973551} & {\hspace{-2mm}\scriptsize 0.969932} & {\hspace{-2mm}\scriptsize 0.969316} & {\hspace{-2mm}\scriptsize 0.969289} & {\hspace{-2mm}\scriptsize 0.969289} & {\hspace{-2mm}\scriptsize 0.969289} & {\hspace{-2mm}\scriptsize 0.969289} & \\ 
\hline 
\multirow{2}{*}{S2} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.4297} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999037} & {\hspace{-2mm}\scriptsize 0.998101} & {\hspace{-2mm}\scriptsize 0.997181} & {\hspace{-2mm}\scriptsize 0.996324} & {\hspace{-2mm}\scriptsize 0.995830} & {\hspace{-2mm}\scriptsize 0.995733} & {\hspace{-2mm}\scriptsize 0.995704} & {\hspace{-2mm}\scriptsize 0.995703} & {\hspace{-2mm}\scriptsize 0.995703} & {\hspace{-2mm}\scriptsize 0.995703} & \\ 
\hline 
\multirow{2}{*}{S3} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{4.9820} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.988811} & {\hspace{-2mm}\scriptsize 0.977912} & {\hspace{-2mm}\scriptsize 0.967047} & {\hspace{-2mm}\scriptsize 0.957582} & {\hspace{-2mm}\scriptsize 0.952109} & {\hspace{-2mm}\scriptsize 0.950310} & {\hspace{-2mm}\scriptsize 0.950181} & {\hspace{-2mm}\scriptsize 0.950180} & {\hspace{-2mm}\scriptsize 0.950180} & {\hspace{-2mm}\scriptsize 0.950180} & \\ 
\hline 
\multirow{2}{*}{S4} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{4.9958} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.989693} & {\hspace{-2mm}\scriptsize 0.979418} & {\hspace{-2mm}\scriptsize 0.969146} & {\hspace{-2mm}\scriptsize 0.958875} & {\hspace{-2mm}\scriptsize 0.950128} & {\hspace{-2mm}\scriptsize 0.950060} & {\hspace{-2mm}\scriptsize 0.950042} & {\hspace{-2mm}\scriptsize 0.950042} & {\hspace{-2mm}\scriptsize 0.950042} & {\hspace{-2mm}\scriptsize 0.950042} & \\ 
\hline 
\multirow{2}{*}{S5} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.1276} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999744} & {\hspace{-2mm}\scriptsize 0.999489} & {\hspace{-2mm}\scriptsize 0.999233} & {\hspace{-2mm}\scriptsize 0.998979} & {\hspace{-2mm}\scriptsize 0.998724} & {\hspace{-2mm}\scriptsize 0.998724} & {\hspace{-2mm}\scriptsize 0.998724} & {\hspace{-2mm}\scriptsize 0.998724} & {\hspace{-2mm}\scriptsize 0.998724} & {\hspace{-2mm}\scriptsize 0.998724} & \\ 
\hline 
\multirow{2}{*}{S6} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.81 & 1.1 & 1.3 & 1.6 & 1.9 & 2.2 & 2.4 & 2.7 & \multirow{2}{*}{0.2597} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999467} & {\hspace{-2mm}\scriptsize 0.998933} & {\hspace{-2mm}\scriptsize 0.998400} & {\hspace{-2mm}\scriptsize 0.997867} & {\hspace{-2mm}\scriptsize 0.997403} & {\hspace{-2mm}\scriptsize 0.997403} & {\hspace{-2mm}\scriptsize 0.997403} & {\hspace{-2mm}\scriptsize 0.997403} & {\hspace{-2mm}\scriptsize 0.997403} & {\hspace{-2mm}\scriptsize 0.997403} & \\ 
\hline 
\multirow{2}{*}{S7} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.0966} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999807} & {\hspace{-2mm}\scriptsize 0.999614} & {\hspace{-2mm}\scriptsize 0.999420} & {\hspace{-2mm}\scriptsize 0.999227} & {\hspace{-2mm}\scriptsize 0.999034} & {\hspace{-2mm}\scriptsize 0.999034} & {\hspace{-2mm}\scriptsize 0.999034} & {\hspace{-2mm}\scriptsize 0.999034} & {\hspace{-2mm}\scriptsize 0.999034} & {\hspace{-2mm}\scriptsize 0.999034} & \\ 
\hline 
\multirow{2}{*}{S8} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.1535} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999693} & {\hspace{-2mm}\scriptsize 0.999386} & {\hspace{-2mm}\scriptsize 0.999079} & {\hspace{-2mm}\scriptsize 0.998772} & {\hspace{-2mm}\scriptsize 0.998465} & {\hspace{-2mm}\scriptsize 0.998465} & {\hspace{-2mm}\scriptsize 0.998465} & {\hspace{-2mm}\scriptsize 0.998465} & {\hspace{-2mm}\scriptsize 0.998465} & {\hspace{-2mm}\scriptsize 0.998465} & \\ 
\hline 
\multirow{2}{*}{S9} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.81 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{3.6622} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.991311} & {\hspace{-2mm}\scriptsize 0.982622} & {\hspace{-2mm}\scriptsize 0.973933} & {\hspace{-2mm}\scriptsize 0.965252} & {\hspace{-2mm}\scriptsize 0.963378} & {\hspace{-2mm}\scriptsize 0.963378} & {\hspace{-2mm}\scriptsize 0.963378} & {\hspace{-2mm}\scriptsize 0.963378} & {\hspace{-2mm}\scriptsize 0.963378} & {\hspace{-2mm}\scriptsize 0.963378} & \\ 
\hline 
\multirow{2}{*}{S10} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.4 & 2.7 & \multirow{2}{*}{0.0905} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999816} & {\hspace{-2mm}\scriptsize 0.999632} & {\hspace{-2mm}\scriptsize 0.999447} & {\hspace{-2mm}\scriptsize 0.999263} & {\hspace{-2mm}\scriptsize 0.999095} & {\hspace{-2mm}\scriptsize 0.999095} & {\hspace{-2mm}\scriptsize 0.999095} & {\hspace{-2mm}\scriptsize 0.999095} & {\hspace{-2mm}\scriptsize 0.999095} & {\hspace{-2mm}\scriptsize 0.999095} & \\ 
\hline 
\multirow{2}{*}{S11} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.3502} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999280} & {\hspace{-2mm}\scriptsize 0.998579} & {\hspace{-2mm}\scriptsize 0.997878} & {\hspace{-2mm}\scriptsize 0.997178} & {\hspace{-2mm}\scriptsize 0.996521} & {\hspace{-2mm}\scriptsize 0.996499} & {\hspace{-2mm}\scriptsize 0.996498} & {\hspace{-2mm}\scriptsize 0.996498} & {\hspace{-2mm}\scriptsize 0.996498} & {\hspace{-2mm}\scriptsize 0.996498} & \\ 
\hline 
\multirow{2}{*}{S12} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.1966} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999585} & {\hspace{-2mm}\scriptsize 0.999169} & {\hspace{-2mm}\scriptsize 0.998754} & {\hspace{-2mm}\scriptsize 0.998339} & {\hspace{-2mm}\scriptsize 0.998035} & {\hspace{-2mm}\scriptsize 0.998034} & {\hspace{-2mm}\scriptsize 0.998034} & {\hspace{-2mm}\scriptsize 0.998034} & {\hspace{-2mm}\scriptsize 0.998034} & {\hspace{-2mm}\scriptsize 0.998034} & \\ 
\hline 
\multirow{2}{*}{S13} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.1275} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999745} & {\hspace{-2mm}\scriptsize 0.999490} & {\hspace{-2mm}\scriptsize 0.999235} & {\hspace{-2mm}\scriptsize 0.998979} & {\hspace{-2mm}\scriptsize 0.998725} & {\hspace{-2mm}\scriptsize 0.998725} & {\hspace{-2mm}\scriptsize 0.998725} & {\hspace{-2mm}\scriptsize 0.998725} & {\hspace{-2mm}\scriptsize 0.998725} & {\hspace{-2mm}\scriptsize 0.998725} & \\ 
\hline 
\multirow{2}{*}{S14} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.1376} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999725} & {\hspace{-2mm}\scriptsize 0.999449} & {\hspace{-2mm}\scriptsize 0.999174} & {\hspace{-2mm}\scriptsize 0.998899} & {\hspace{-2mm}\scriptsize 0.998624} & {\hspace{-2mm}\scriptsize 0.998624} & {\hspace{-2mm}\scriptsize 0.998624} & {\hspace{-2mm}\scriptsize 0.998624} & {\hspace{-2mm}\scriptsize 0.998624} & {\hspace{-2mm}\scriptsize 0.998624} & \\ 
\hline 
\multirow{2}{*}{S15} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.81 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.4 & 2.7 & \multirow{2}{*}{0.5168} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.998826} & {\hspace{-2mm}\scriptsize 0.997686} & {\hspace{-2mm}\scriptsize 0.996560} & {\hspace{-2mm}\scriptsize 0.995532} & {\hspace{-2mm}\scriptsize 0.994927} & {\hspace{-2mm}\scriptsize 0.994857} & {\hspace{-2mm}\scriptsize 0.994832} & {\hspace{-2mm}\scriptsize 0.994832} & {\hspace{-2mm}\scriptsize 0.994832} & {\hspace{-2mm}\scriptsize 0.994832} & \\ 
\hline 
\multirow{2}{*}{S16} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.0711} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999858} & {\hspace{-2mm}\scriptsize 0.999716} & {\hspace{-2mm}\scriptsize 0.999573} & {\hspace{-2mm}\scriptsize 0.999431} & {\hspace{-2mm}\scriptsize 0.999289} & {\hspace{-2mm}\scriptsize 0.999289} & {\hspace{-2mm}\scriptsize 0.999289} & {\hspace{-2mm}\scriptsize 0.999289} & {\hspace{-2mm}\scriptsize 0.999289} & {\hspace{-2mm}\scriptsize 0.999289} & \\ 
\hline 
\multirow{2}{*}{S17} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.0936} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999813} & {\hspace{-2mm}\scriptsize 0.999625} & {\hspace{-2mm}\scriptsize 0.999438} & {\hspace{-2mm}\scriptsize 0.999251} & {\hspace{-2mm}\scriptsize 0.999064} & {\hspace{-2mm}\scriptsize 0.999064} & {\hspace{-2mm}\scriptsize 0.999064} & {\hspace{-2mm}\scriptsize 0.999064} & {\hspace{-2mm}\scriptsize 0.999064} & {\hspace{-2mm}\scriptsize 0.999064} & \\ 
\hline 
\multirow{2}{*}{S18} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.0701} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999860} & {\hspace{-2mm}\scriptsize 0.999719} & {\hspace{-2mm}\scriptsize 0.999579} & {\hspace{-2mm}\scriptsize 0.999439} & {\hspace{-2mm}\scriptsize 0.999299} & {\hspace{-2mm}\scriptsize 0.999299} & {\hspace{-2mm}\scriptsize 0.999299} & {\hspace{-2mm}\scriptsize 0.999299} & {\hspace{-2mm}\scriptsize 0.999299} & {\hspace{-2mm}\scriptsize 0.999299} & \\ 
\hline 
\multirow{2}{*}{S19} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.0837} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999832} & {\hspace{-2mm}\scriptsize 0.999665} & {\hspace{-2mm}\scriptsize 0.999497} & {\hspace{-2mm}\scriptsize 0.999330} & {\hspace{-2mm}\scriptsize 0.999163} & {\hspace{-2mm}\scriptsize 0.999163} & {\hspace{-2mm}\scriptsize 0.999163} & {\hspace{-2mm}\scriptsize 0.999163} & {\hspace{-2mm}\scriptsize 0.999163} & {\hspace{-2mm}\scriptsize 0.999163} & \\ 
\hline 
\multirow{2}{*}{S20} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.1785} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999643} & {\hspace{-2mm}\scriptsize 0.999286} & {\hspace{-2mm}\scriptsize 0.998929} & {\hspace{-2mm}\scriptsize 0.998571} & {\hspace{-2mm}\scriptsize 0.998215} & {\hspace{-2mm}\scriptsize 0.998215} & {\hspace{-2mm}\scriptsize 0.998215} & {\hspace{-2mm}\scriptsize 0.998215} & {\hspace{-2mm}\scriptsize 0.998215} & {\hspace{-2mm}\scriptsize 0.998215} & \\ 
\hline 
\multirow{2}{*}{S21} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.1202} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999760} & {\hspace{-2mm}\scriptsize 0.999519} & {\hspace{-2mm}\scriptsize 0.999279} & {\hspace{-2mm}\scriptsize 0.999038} & {\hspace{-2mm}\scriptsize 0.998798} & {\hspace{-2mm}\scriptsize 0.998798} & {\hspace{-2mm}\scriptsize 0.998798} & {\hspace{-2mm}\scriptsize 0.998798} & {\hspace{-2mm}\scriptsize 0.998798} & {\hspace{-2mm}\scriptsize 0.998798} & \\ 
\hline 
\multirow{2}{*}{S22} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.0792} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999842} & {\hspace{-2mm}\scriptsize 0.999683} & {\hspace{-2mm}\scriptsize 0.999525} & {\hspace{-2mm}\scriptsize 0.999367} & {\hspace{-2mm}\scriptsize 0.999208} & {\hspace{-2mm}\scriptsize 0.999208} & {\hspace{-2mm}\scriptsize 0.999208} & {\hspace{-2mm}\scriptsize 0.999208} & {\hspace{-2mm}\scriptsize 0.999208} & {\hspace{-2mm}\scriptsize 0.999208} & \\ 
\hline 
\multirow{2}{*}{S23} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.2896} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999376} & {\hspace{-2mm}\scriptsize 0.998752} & {\hspace{-2mm}\scriptsize 0.998129} & {\hspace{-2mm}\scriptsize 0.997505} & {\hspace{-2mm}\scriptsize 0.997116} & {\hspace{-2mm}\scriptsize 0.997104} & {\hspace{-2mm}\scriptsize 0.997104} & {\hspace{-2mm}\scriptsize 0.997104} & {\hspace{-2mm}\scriptsize 0.997104} & {\hspace{-2mm}\scriptsize 0.997104} & \\ 
\hline 
\multirow{2}{*}{S24} & $\Delta $ & 0.0 & 0.27 & 0.53 & 0.8 & 1.1 & 1.3 & 1.6 & 1.9 & 2.1 & 2.4 & 2.7 & \multirow{2}{*}{0.0589} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999882} & {\hspace{-2mm}\scriptsize 0.999764} & {\hspace{-2mm}\scriptsize 0.999646} & {\hspace{-2mm}\scriptsize 0.999528} & {\hspace{-2mm}\scriptsize 0.999411} & {\hspace{-2mm}\scriptsize 0.999411} & {\hspace{-2mm}\scriptsize 0.999411} & {\hspace{-2mm}\scriptsize 0.999411} & {\hspace{-2mm}\scriptsize 0.999411} & {\hspace{-2mm}\scriptsize 0.999411} & \\ 
\hline 
\multirow{2}{*}{S25} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.4 & 2.7 & \multirow{2}{*}{0.9145} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.998130} & {\hspace{-2mm}\scriptsize 0.996280} & {\hspace{-2mm}\scriptsize 0.994435} & {\hspace{-2mm}\scriptsize 0.992594} & {\hspace{-2mm}\scriptsize 0.991023} & {\hspace{-2mm}\scriptsize 0.990874} & {\hspace{-2mm}\scriptsize 0.990856} & {\hspace{-2mm}\scriptsize 0.990855} & {\hspace{-2mm}\scriptsize 0.990855} & {\hspace{-2mm}\scriptsize 0.990855} & \\ 
\hline 
\multirow{2}{*}{S26} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{1.9237} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.996136} & {\hspace{-2mm}\scriptsize 0.992416} & {\hspace{-2mm}\scriptsize 0.988744} & {\hspace{-2mm}\scriptsize 0.985215} & {\hspace{-2mm}\scriptsize 0.982117} & {\hspace{-2mm}\scriptsize 0.981046} & {\hspace{-2mm}\scriptsize 0.980792} & {\hspace{-2mm}\scriptsize 0.980763} & {\hspace{-2mm}\scriptsize 0.980763} & {\hspace{-2mm}\scriptsize 0.980763} & \\ 
\hline 
\multirow{2}{*}{S27} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.0291} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999937} & {\hspace{-2mm}\scriptsize 0.999876} & {\hspace{-2mm}\scriptsize 0.999815} & {\hspace{-2mm}\scriptsize 0.999756} & {\hspace{-2mm}\scriptsize 0.999717} & {\hspace{-2mm}\scriptsize 0.999712} & {\hspace{-2mm}\scriptsize 0.999709} & {\hspace{-2mm}\scriptsize 0.999709} & {\hspace{-2mm}\scriptsize 0.999709} & {\hspace{-2mm}\scriptsize 0.999709} & \\ 
\hline 
\multirow{2}{*}{S28} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.0383} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999918} & {\hspace{-2mm}\scriptsize 0.999838} & {\hspace{-2mm}\scriptsize 0.999758} & {\hspace{-2mm}\scriptsize 0.999681} & {\hspace{-2mm}\scriptsize 0.999629} & {\hspace{-2mm}\scriptsize 0.999619} & {\hspace{-2mm}\scriptsize 0.999617} & {\hspace{-2mm}\scriptsize 0.999617} & {\hspace{-2mm}\scriptsize 0.999617} & {\hspace{-2mm}\scriptsize 0.999617} & \\ 
\hline 
\multirow{2}{*}{S29} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{2.4903} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.994427} & {\hspace{-2mm}\scriptsize 0.989243} & {\hspace{-2mm}\scriptsize 0.984136} & {\hspace{-2mm}\scriptsize 0.979593} & {\hspace{-2mm}\scriptsize 0.976510} & {\hspace{-2mm}\scriptsize 0.975367} & {\hspace{-2mm}\scriptsize 0.975113} & {\hspace{-2mm}\scriptsize 0.975097} & {\hspace{-2mm}\scriptsize 0.975097} & {\hspace{-2mm}\scriptsize 0.975097} & \\ 
\hline 
\multirow{2}{*}{S30} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.6388} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.998594} & {\hspace{-2mm}\scriptsize 0.997207} & {\hspace{-2mm}\scriptsize 0.995825} & {\hspace{-2mm}\scriptsize 0.994515} & {\hspace{-2mm}\scriptsize 0.993720} & {\hspace{-2mm}\scriptsize 0.993629} & {\hspace{-2mm}\scriptsize 0.993613} & {\hspace{-2mm}\scriptsize 0.993612} & {\hspace{-2mm}\scriptsize 0.993612} & {\hspace{-2mm}\scriptsize 0.993612} & \\ 
\hline 
\multirow{2}{*}{S31} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{9.2232} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.979913} & {\hspace{-2mm}\scriptsize 0.961560} & {\hspace{-2mm}\scriptsize 0.943645} & {\hspace{-2mm}\scriptsize 0.926758} & {\hspace{-2mm}\scriptsize 0.914358} & {\hspace{-2mm}\scriptsize 0.909108} & {\hspace{-2mm}\scriptsize 0.907796} & {\hspace{-2mm}\scriptsize 0.907768} & {\hspace{-2mm}\scriptsize 0.907768} & {\hspace{-2mm}\scriptsize 0.907768} & \\ 
\hline 
\multirow{2}{*}{S32} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{2.3555} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.994752} & {\hspace{-2mm}\scriptsize 0.990314} & {\hspace{-2mm}\scriptsize 0.986136} & {\hspace{-2mm}\scriptsize 0.982095} & {\hspace{-2mm}\scriptsize 0.978792} & {\hspace{-2mm}\scriptsize 0.977042} & {\hspace{-2mm}\scriptsize 0.976475} & {\hspace{-2mm}\scriptsize 0.976445} & {\hspace{-2mm}\scriptsize 0.976445} & {\hspace{-2mm}\scriptsize 0.976445} & \\ 
\hline 
\multirow{2}{*}{S33} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.8485} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.998103} & {\hspace{-2mm}\scriptsize 0.996229} & {\hspace{-2mm}\scriptsize 0.994361} & {\hspace{-2mm}\scriptsize 0.992696} & {\hspace{-2mm}\scriptsize 0.991606} & {\hspace{-2mm}\scriptsize 0.991530} & {\hspace{-2mm}\scriptsize 0.991517} & {\hspace{-2mm}\scriptsize 0.991515} & {\hspace{-2mm}\scriptsize 0.991515} & {\hspace{-2mm}\scriptsize 0.991515} & \\ 
\hline 
\multirow{2}{*}{S34} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.1375} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999695} & {\hspace{-2mm}\scriptsize 0.999411} & {\hspace{-2mm}\scriptsize 0.999136} & {\hspace{-2mm}\scriptsize 0.998880} & {\hspace{-2mm}\scriptsize 0.998710} & {\hspace{-2mm}\scriptsize 0.998647} & {\hspace{-2mm}\scriptsize 0.998627} & {\hspace{-2mm}\scriptsize 0.998625} & {\hspace{-2mm}\scriptsize 0.998625} & {\hspace{-2mm}\scriptsize 0.998625} & \\ 
\hline 
\multirow{2}{*}{S35} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.1056} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999767} & {\hspace{-2mm}\scriptsize 0.999544} & {\hspace{-2mm}\scriptsize 0.999322} & {\hspace{-2mm}\scriptsize 0.999128} & {\hspace{-2mm}\scriptsize 0.998980} & {\hspace{-2mm}\scriptsize 0.998951} & {\hspace{-2mm}\scriptsize 0.998945} & {\hspace{-2mm}\scriptsize 0.998944} & {\hspace{-2mm}\scriptsize 0.998944} & {\hspace{-2mm}\scriptsize 0.998944} & \\ 
\hline 
\multirow{2}{*}{S36} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{1.5463} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.996632} & {\hspace{-2mm}\scriptsize 0.993362} & {\hspace{-2mm}\scriptsize 0.990135} & {\hspace{-2mm}\scriptsize 0.987283} & {\hspace{-2mm}\scriptsize 0.985292} & {\hspace{-2mm}\scriptsize 0.984667} & {\hspace{-2mm}\scriptsize 0.984548} & {\hspace{-2mm}\scriptsize 0.984537} & {\hspace{-2mm}\scriptsize 0.984537} & {\hspace{-2mm}\scriptsize 0.984537} & \\ 
\hline 
\multirow{2}{*}{S37} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{3.3147} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.993184} & {\hspace{-2mm}\scriptsize 0.986403} & {\hspace{-2mm}\scriptsize 0.979636} & {\hspace{-2mm}\scriptsize 0.972950} & {\hspace{-2mm}\scriptsize 0.967465} & {\hspace{-2mm}\scriptsize 0.966906} & {\hspace{-2mm}\scriptsize 0.966854} & {\hspace{-2mm}\scriptsize 0.966853} & {\hspace{-2mm}\scriptsize 0.966853} & {\hspace{-2mm}\scriptsize 0.966853} & \\ 
\hline 
\multirow{2}{*}{S38} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{1.1891} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.997604} & {\hspace{-2mm}\scriptsize 0.995296} & {\hspace{-2mm}\scriptsize 0.993000} & {\hspace{-2mm}\scriptsize 0.990749} & {\hspace{-2mm}\scriptsize 0.988826} & {\hspace{-2mm}\scriptsize 0.988223} & {\hspace{-2mm}\scriptsize 0.988127} & {\hspace{-2mm}\scriptsize 0.988109} & {\hspace{-2mm}\scriptsize 0.988109} & {\hspace{-2mm}\scriptsize 0.988109} & \\ 
\hline 
\multirow{2}{*}{S39} & $\Delta $ & 0.0 & 0.27 & 0.55 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.2431} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999468} & {\hspace{-2mm}\scriptsize 0.998939} & {\hspace{-2mm}\scriptsize 0.998411} & {\hspace{-2mm}\scriptsize 0.997904} & {\hspace{-2mm}\scriptsize 0.997589} & {\hspace{-2mm}\scriptsize 0.997571} & {\hspace{-2mm}\scriptsize 0.997569} & {\hspace{-2mm}\scriptsize 0.997569} & {\hspace{-2mm}\scriptsize 0.997569} & {\hspace{-2mm}\scriptsize 0.997569} & \\ 
\hline 
\multirow{2}{*}{S40} & $\Delta $ & 0.0 & 0.27 & 0.54 & 0.82 & 1.1 & 1.4 & 1.6 & 1.9 & 2.2 & 2.5 & 2.7 & \multirow{2}{*}{0.1763} \\ 
& $Z^*$ & {\hspace{-2mm}\scriptsize 1.000000} & {\hspace{-2mm}\scriptsize 0.999629} & {\hspace{-2mm}\scriptsize 0.999275} & {\hspace{-2mm}\scriptsize 0.998930} & {\hspace{-2mm}\scriptsize 0.998602} & {\hspace{-2mm}\scriptsize 0.998350} & {\hspace{-2mm}\scriptsize 0.998247} & {\hspace{-2mm}\scriptsize 0.998238} & {\hspace{-2mm}\scriptsize 0.998237} & {\hspace{-2mm}\scriptsize 0.998237} & {\hspace{-2mm}\scriptsize 0.998237} & \\ 
	\hline \hline 
	%\end{tabular}
\caption{\small Delta values and optimal values of the price optimization problem with robust optimization
	approach. \label{tbl:deltaoptval}}
%\end{table}
\end{longtable}
\end{center}
\end{landscape}
